Control-Tree Optimization: an approach to MPC under discrete Partial Observability

This paper presents a new approach to Model Predictive Control for environments where essential, discrete variables are partially observed. Under this assumption, the belief state is a probability distribution over a finite number of states. We optimize a \textit{control-tree} where each branch assumes a given state-hypothesis. The control-tree optimization uses the probabilistic belief state information. This leads to policies more optimized with respect to likely states than unlikely ones, while still guaranteeing robust constraint satisfaction at all times. We apply the method to both linear and non-linear MPC with constraints. The optimization of the \textit{control-tree} is decomposed into optimization subproblems that are solved in parallel leading to good scalability for high number of state-hypotheses. We demonstrate the real-time feasibility of the algorithm on two examples and show the benefits compared to a classical MPC scheme optimizing w.r.t. one single hypothesis.

==> removed_bib <==

@article{ad-1,
author = {Cesari, Gianluca and Schildbach, Georg and Carvalho, Ashwin and Borrelli, Francesco},
year = {2017},
month = {10},
pages = {23-35},
title = {\href{https://ieeexplore.ieee.org/document/7990647}{Scenario Model Predictive Control for Lane Change Assistance and Autonomous Driving on Highways}},
volume = {9},
journal = {IEEE Intelligent Transportation Systems Magazine},
doi = {10.1109/mits.2017.2709782}
}

@inproceedings{ad-2,
author = {Bruedigam, Tim and Olbrich, Michael and Leibold, Marion and Wollherr, Dirk},
year = {2018},
month = {11},
pages = {1317-1324},
title = {\href{https://www.researchgate.net/publication/329612249_Combining_Stochastic_and_Scenario_Model_Predictive_Control_to_Handle_Target_Vehicle_Uncertainty_in_an_Autonomous_Driving_Highway_Scenario}{Combining Stochastic and Scenario Model Predictive Control to Handle Target Vehicle Uncertainty in an Autonomous Driving Highway Scenario}},
doi = {10.1109/ITSC.2018.8569909}
}

